Recursive definitions on surreal numbers

Let No be Conway's class of surreal numbers. I will make explicit the notion of a function f on No recursively defined over some family of functions. Under some "tameness" and uniformity condition, f must satisfy some interesting properties; in particular, the supremum of the class of element greater or equal to a fixed d in No is actually an element of No. For similar reasons, the concatenation function x:y cannot be defined recursively in a uniform way over polynomial functions.

==> ondue.tex <==
\section{Recursive definitions on Nimbers}
%
\subsection{\Ont}
The class $\Ont$ of{} `nimbers' was described in \cite{conway}.
It can be identified with the class $\On$ of ordinals.
I will show that theorems analogous to the ones proved here for $\On$ are valid in $\Ont$.
\begin{definizione}
A nimber $x$ is strictly simpler than a nimber $y$ iff, as ordinal numbers,
$x<y$.
\end{definizione}
By definition, given any non-empty class of nimbers $S$, there is a simplest element in it.
\begin{definizione}
Let $L$ be a subclass of $\Ont$.
$\cutn{L}$ is the simplest element in $\Ont$ not $L$ (if $L \neq \Ont$)\footnote{Conway used the notations $\mex{L}$ instead of $\cutn{L}$, and $\Ccut{L}{R}$ instead of $\cut{L}{R}$.
But I think that similar concepts should use similar notations.}.
\end{definizione}
Note that if $L$ is a set then $\cutn{L}$ is always defined.

If $x=\cutn{L}$, an element $\xo$ of $L$ is an option of $x$.
$x=\cutn{y:y<x}$ is the canonical representation of $x$.
%
\subsection{Recursive definitions}
\begin{definizione}[Recursive definitions]
Let $\ff:\Ont\to\Ont$ be a function, let $L$ be a set of functions.
I write
\[
\ff = \cutn{L}
\]
iff for all $x\in\Ont$
\be\label{eq:recdeft}
\ff(x) = \cutn{\ffo\paren{x,\xo,\ff(\xo)}},
\ee
where $\xo$ varies among the canonical options of $x$, and $\ffo$ varies in $L$.
\end{definizione}
The formula~\ref{eq:recdeft} gives a recursive definition of $\ff$.

Note that this notion of recursive definition is more restrictive than the usual notion of function defined by recursion on $\On$.
\begin{definizione}
The recursive definition $\ff=\cutn{\ffo}$ is uniform if the value of $\ff(x)$ does not depend on the chosen representation of $x$.
This means that:
\begin{itemize}
\item $\forall x,y\in\Ont$ such that $x\neq y$
\[
\ffo\Paren{x,y,\ff(y)} \neq \ff(x).
\]
\item If $x\in\Ont$ and $x=\cutn{L}$ is the canonical representation of $x$, then
\[
\ff(x) = \cutn{\ffo\paren{x,\xo,\ff(\xo)}},
\]
where $\xo$ varies in $L$.
\end{itemize}
\end{definizione}
If $\Afam$ is a family of functions, and $\ff:\Ont\to\Ont$, then $f$ is (\emph{uniformly}) \emph{recursive} over $\Afam$ iff there exists  a subset $L$ of $\Afam$ such that $\ff=\cutn{L}$ is a (uniform) recursive definition of $\ff$.

Similar definitions can be given for functions of many variables, along the lines of \S\ref{sec:manyVars}.
%
\subsection{Algebraic structure of \Ont}
%
\begin{example}
Conway gives the recursive definitions of the sum and product of nimbers:
\[\begin{aligned}
x+y &= \cutn{\xo+y,x+\yo}\\
-x  &= \cutn{-\xo}\\
xy  &= \cutn{\xo y + x \yo - \xo\yo}.
\end{aligned}\]
\end{example}
With the previous definitions, $\Ont$ is an algebraically closed field of characteristic $2$.
Note that $-x=x$.

$0$ is the neutral element of addition, $1$ is the unit element.
Therefore, the set $\set{0,1}$ is the subfield of $\Ont$ with $2$ elements.

The order $\leq$ on $\Ont$ induces the lexicographic order on $\Ont[x]$, with higher degree coefficients more important than lower degree ones.
With this order, $\Ont[x]$ is a well order.
%
\subsection{Main results}
%
For the rest of this section, $\Afam$ will be some family of functions on  $\Ont$.
\begin{definizione}
A subclass $S$ of $\Ont$ is initial iff 
\[
\forall x\in S\ \forall y\in\Ont\ y<x\to y\in S
\]
\end{definizione}
Note that the initial subclasses of $\Ont$ are all $\Ont$ or ordinals (under the identification of an ordinal with the set of smaller ordinals).

The definitions of the closure of $S$ under $\Afam$, $\closA{S}$, and of the closure of $S$ under solutions of $\Afam$ are analogous to the ones in \S\ref{sec:results}.
\begin{lemma}\label{lem:initialN}
Let $S\subseteq\No$ be an initial subclass of $\No$, $L$ be a subclass of $S$,
$x:=\cutn{L}$ (if it exists).
Let $z<x$.
Then, $z\in S$.
\end{lemma}
\begin{proof}
$x$ is the smallest element not in $L$ and $z<x$, therefore $z\in L\subseteq S$.
\end{proof}
The following is the analogous of Theorem~\ref{thm:initial}.
\begin{thm}\label{thm:initialN}
Suppose that for every $T\subseteq\Ont$ initial $\closA{T}$ is also initial.
Let $\ff:\Ont^n\to\Ont$ be recursive over $\Afam$.
Let $S_1,\dotsc,S_n$ be initial subclasses of $\Ont$, 
$S:=S_1\times\dotsb\times S_n$.
Then, $\closA{\Paren{S_1\cup\dotsb\cup S_n\cup\ff(S)}}$ is also initial.

Moreover, if every $\ffo$ option of $\ff$ is function only of $\ff(\xo)$, 
then $\closA{\paren{\ff(S)}}$ is initial.
\end{thm}
\begin{proof}
Repeat word-by-word the proof of  Theorem~\ref{thm:initial}, using Lemma~\ref{lem:initialN} instead of~\ref{lem:initial}.
\end{proof}
Theorem~\ref{thm:initialCl} is also valid in this context (with the obvious modifications), with exactly the same proof.
Therefore, also the Corollaries~\ref{cor:initial} and~\ref{cor:Kx} are true.
\begin{corollary}\label{cor:initialN}
Let $S,U$ be initial subclasses of $\Ont$. 
Then, the following subclasses of $\Ont$ are also initial:
\begin{enumerate}
\item The (additive) subgroup generated by $S$.
\item The subring generated by $S$ .
\item $-S :=\set{-x: x\in S}$.
\item $S+U := \set{x+y: x\in S, y\in U}$.
\item The subgroup generated by $SU:=\set{xy: x\in S, y\in U}$.
\end{enumerate}
\end{corollary}
\begin{corollary}
Let $\Kfield$ be an initial subring of $\Ont$.
Let $L$ be a subset of $\Kfield$, and let $c:=\cutn{L}$.
Then, $\Kfield[c]$ is also an initial subring of $\Ont$.
\end{corollary}
Similar results were already proved in \cite{conway}.

To state the other theorems in this context, I need a notion of tameness.
\begin{definizione}
Let $\ff:\Ont^{n+1}\to\Ont$, $\bv\in\Ont^n$.
\[
\Zero{\ff,\bv} := \set{x\in\Ont: \ff(x,\bv)=0}.
\]

$\ff$ is \emph{tame} iff for every $\bv\in\Ont^n$ either $\ff(x,\bv)$ is constant, or for all $d\in\Ont$ $\Zero{\ff-d,\bv}$ is a proper \emph{set}.
\end{definizione}
In particular, any polynomial function and any injective function are tame (because $\Zero{\ff-d,\bv}$ is finite).
\begin{example}
Let
\[
\ff(x) = \cutn{0,x}.
\]
The definition of $\ff$ is uniform.
Moreover,
\[
\ff(x) = 
\begin{cases}
1 &\text{iff } x=0\\
0 &\text{otherwise.}
\end{cases}\]
Therefore, $\ff$ is not tame.
\end{example}
%
It is possible to state an analogous of Theorem~\ref{thm:sup} in this context, and apply it (togetehr with induction on $\Ont$) to obtain that $\Ont$ is an algebraicallly closed field, but it does not seem worthwhile, due to its lack of generality.
%The following is the analogous of Theorem~\ref{thm:sup}.
%\begin{thm}\label{thm:supN}
%Suppose that $\Afam$ is tame.
%Let $\ff:\Ont\to\Ont$ be uniformly recursive over $\Afam$ and tame.
%
%Then, either $\ff$ is constant or for every $d\in\Ont$ $\Zero{\ff-d}$ is non-empty (\ie $\ff$ is surjective) .
%\end{thm}
%Note that the only hypothesis on $\Afam$ is its tameness.
%\begin{proof}
%I construct a $L$ subset of $\Ont$ such that $c:=\cutn{L}$ and $\ff(c)=d$.
%
%$\ff(c)=d$ is equivalent to
%\begin{subequations}\begin{align}
%\ff(c) &\neq\Do \label{eq:optN1}\\
%\ffo(c,\co,\ff(\co)) &\neq d\label{eq:optN2}.
%\end{align}\end{subequations}
%
%\eqref{eq:optN1}
%It is enough that $L$ contains the set $\Zero{\ff-\Do}$.
%
%\eqref{eq:optN2}
%Let $\co$ be an `old' option of $c$.
%Add to $L$ the set $\Zero{\ffo-d,(\co,\ff(\co)}$.
%
%At the end of this process, $\ff(c)=d$.
%\end{proof}
%Note that the previous proof is \emph{not} done by induction on $d$.
%
%In \cite{conway} Conway proves first that $\Ont$ is a domain of characteristic $2$, then that it is an algebraically closed field.

%To obtain the same result, we can use the fact that $\Ont$ is a domain, and apply the theorem~\ref{thm:supN} and induction on $\Ont[x]$.
%
Now, the analogue of Theorem~\ref{thm:closSol}.
\begin{thm}\label{thm:closSolN}
Suppose that $\Afam$ is tame.
Let $\ff:\Ont\to\Ont$ uniformly recursive over $\Afam$ and tame.

Suppose that for every $S$ initial subclass of $\Ont$, the closure of $S$ under solutions of $\Afam$ and under $\ff$ is also initial.
Then, the closure of $S$ under solutions of $\Afamf$ is initial.
\end{thm}
%The proof is quite similar to the one of theorem~\ref{thm:sup}.
\begin{proof}
Let $T$ be the maximal initial subclass of the closure of $S$ under solutions of $\Afamf$.
By hypothesis, $T$ is closed under solutions of $\Afam$ and under $\ff$.
Therefore, it is enough to prove that $T$ is closed under solutions of $\ff$.
If $\ff$ is constant, there is nothing to prove.
Otherwise, let $d\in T$, $c\in\No$ such that $\ff(c) =d$.
I will prove that $c\in T$ by induction on $d$.

I will give $L\subseteq T$ options of $c$.

Assume that $\ff=\cutn{\ffo}$.
Then, $\ff(c)=d$ is equivalent to
\begin{subequations}
  \begin{align}
    \label{eq:zeroN1}
    \Do&\neq\ff(c)\\
    \label{eq:zeroN2}
    \ffo(c,\co,\ff(\co))&\neq d.
  \end{align}
\end{subequations}

\eqref{eq:zeroN1}
$\Do<d$ and $d\in T$, therefore $\Do\in T$, and, by inductive hypothesis, $\Zero{\ff-\Do}\subseteq T$.
Therefore, it is enough to add to $L$ the set $\Zero{\ff-\Do}$.

\eqref{eq:zeroN2}
Let $\co$ be an `old' option of $c$.
Let $\gf(x) := \ffo(x,\co,\ff(\co))$.
$\co$ and $\ff(\co)$ are in $T$.
\begin{itemize}
\item If $\gf$ is not constant then, by hypothesis on $\Afam$, $\Zero{\gf-d}\subseteq T$.
Therefore I can add to $L$ the set $\Zero{\gf-d}$.
\item If $\gf$ is constant, since $\gf(c)\neq \ff(c)=d$, then $\gf(x)\neq d$, so I do not need to add any `new' options to $L$.
\end{itemize}
At the end of this process, I find $c=\cutn{L}\in T$ such that $\ff(c)=d$.
\end{proof}

The following and other results on the algebraic structure of $\Ont$ are already proved in \cite{conway}.

The following corollary si proved like Corollaries~\ref{cor:initReal} and~\ref{cor:initField} using the field of two elements instead of $\Raz$.
%and theorems are proved like corollaries~\ref{cor:initReal} and~\ref{cor:initField} and theorem~\ref{thm:isomRCF}, using the field of two elements instead of $\Raz$.
\begin{corollary}
The algebraic closure of an initial subring of $\Ont$ is initial.

More in general, let $S$ be an initial subclass of $\Ont$.

Then, the smallest algebraically closed field containing $S$ is initial.

Let $n>0\in\Nat$.
Let $T$ be the smallest subclass of $\Ont$ such that:
\begin{itemize}
\item $T$ contains $S$.
\item $T$ is a ring.
\item $T$ contains the  roots of any non-constant polynomials of degree up to $n$ and coefficients in $T$.
\end{itemize}
Then, $T$ is initial.
In particular, the field generated by $S$ is initial.
\end{corollary}
\begin{example}
For any $\alpha\in\Ont$, let $L(\alpha)$ be the set of all ordinals less than $\alpha$ ($L(\alpha)$ can be identified with $\alpha$ itself if we use von Neumann's convention); note that $\alpha=\cutn{L(\alpha)}$ is the canonical representation of $\alpha$.

For any $n>0\in\Nat$, $L(n)$ is a subfield of $\Ont$ iff $n$ is of the form
$2^{2^m}$ for some $m>0\in\Nat$.

Therefore, $L(\omega)$ is the union of all finite fields $L({2^{2^m}})$, so it is a field and is the quadratic closure of $2$.
So, $\omega$ itself must be a root of the simplest irreducible polynomial of degree $3$ in $\omega[x]$.
\end{example}
%This and much more is proved in \cite{conway}.
The following is the analogue of Theorem~\ref{thm:isomRCF}.
\begin{thm}\label{thm:isomACF}
Let $\Kfield$ be an algebraically closed field of characteristic $2$ and a proper set.
Then, $\Kfield$ is isomorphic to an initial subfield of $\Ont$.
\end{thm}
\begin{example}
$\Ffield_8$, the finite field (of characteristic $2$) with $8$ elements is not isomorphic to an initial subfield of $\Ont$; it contains $\omega$.
\end{example}
%
\subsection{The concatenation function}
%
Let $\ff(x):= x \oplus 1$, where $\oplus$ is the ordinal sum.

Then, $\ff$ is obviously injective, so it is tame.
On the other hand, it is not surjective, because no limit ordinal is in its range.

Let $\Afam$ be the family of polynomial functions over $\Ont$.
Then, $\ff$ is recursive over $\Afam$;
\[
\ff(x) = \cutn{\xo}.
\]
However, the previous definition is not uniform.
An open question: is $\ff$ uniformly recursive over $\Afam$?
My conjecture is that it is not.
%Therefore, by theorem~\ref{thm:supN}, $\ff$ cannot be uniformly recursive over any tame family of functions $\Afam$.
%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "article"
%%% End: 

